Invitation to Local Algorithms

This text provides an introduction to distributed local algorithms -- an area at the intersection of theoretical computer science and discrete mathematics. We collect recent results in the area and demonstrate how they lead to a clean theory. We also discuss many connections of local algorithms to fields such as parallel, distributed, and sublinear algorithms, or descriptive combinatorics.

==> chapter1/25highlights.tex <==



\subsection*{A Few Quick Highlights}

I think it would be nice to mention a few quick highlights of what kind of understanding we have about local complexity and local algorithms. If you have never heard the definitions of 

A maximal independent set is a problem where we are asked to select a bunch of vertices in an input graph so that no two selected vertices are neighboring, but every unselected vertex neighbors with at least one selected vertex. There is a simple sequential algorithm for this problem: Just go over the vertices in an arbitrary order and whenever you can add that vertex to the independent set, do it. It turns out that there is a general framework of turning this sequential local algorithm into a fast distributed local algorithm in which every vertex looks at its small neighborhood and outputs an answer for itself, regardless of how the graph looks like outside of that neighborhood. (See Chapter 1)

We can derandomize most local algorithms with only a small blowup in the local complexity. (See Chapter 2)

We have an amazing theory of what is happening with problems with sublogarithmic complexity in constant degree graphs, we can classify reasonable problems into just three complexity classes, and we know that there are no problems outside of these three classes -- i.e., instead of a dense range of complexities as one would probably expect, we instead see phase transitions. (Chapter )

There are many applications of results in local complexity to distributed algorithms, parallel algorithms, massively parallel algorithms, or local computation algorithms. 

More surprisingly, there is a deep connection between local complexity and descriptive combinatorics (field about certain problems that arise in set theory / measure theory). 

All above results are quite general, but, of course, we have a lot of understanding about many concrete problems -- clusterings (Chapter 3), independent sets, matchings, colorings, etc. (Chapter 4)

==> feedback.tex <==
p 30. Maximal Matching.  Isn't log^{4/3} n for approximate maximum matching?  This is different than maximal matching.  I don't see how this translates into a randomized O(log^{4/3} log n) time guarantee via [Ghaffari]?  You still need log\Delta for graph shattering.

==> preface.tex <==
\chapter*{Preface}

The thesis is organized into two parts. The first part -- \cref{chap:1_local_complexity_fundamentals,chap:2_below_logn,chap:3_concrete_results} -- contains a survey of the past work in the area of local algorithms, also containing some proofs. I wrote it in the hope that I would later add a few pictures and post it online so that it could be helpful, e.g., as a material for reading groups on local algorithms. I would greatly appreciate any feedback on this part of the thesis. 

This first part is divided into three chapters: In \cref{chap:1_local_complexity_fundamentals}, we explain how the theory of local algorithms is extremely clean if we disregard polylogarithmic factors. 
In \cref{chap:2_below_logn}, we put together a number of results in the area to give a more or less self-contained proof of the remarkable classification theorem of local problems with sublogarithmic local complexity on bounded degree graphs. In \cref{chap:3_concrete_results}, we briefly discuss connections and applications of local algorithms to other areas of computer science and discrete mathematics. 

%I understand that such a long introduction is not standard, but since I already had to write one, I thought that I could as well spend a bit more work and create something that could, hopefully, have some additional value. If a member of the doctoral committee plans to read it, I will be grateful for comments on how to improve it. 
\vspace{1em}

The next part of the thesis begins with \cref{chap:5_overview} which overviews some new results related to the area of local algorithms. These results are small pieces fitting into the big picture presented in the first three chapters and in \cref{chap:5_overview}, we discuss how exactly those small pieces fit there. 

The presented technical results are divided into two parts. First, in \cref{chap:6_network_decomposition,chap:7_lll_sharp_threshold,chap:8speedup_logstar}, we focus on results that are related to the fundamental theory of local algorithms. We present three results based on the following three papers:

\cref{chap:6_network_decomposition}  presents results from the following paper:
\begin{adjustwidth}{.1\textwidth}{.1\textwidth}
{
\vspace{1em}
\setlength{\parindent}{0pt}
\bibentry{rozhon_haeupler_grunau2023simple_decomposition}
\vspace{1em}
}
\end{adjustwidth}


\cref{chap:7_lll_sharp_threshold} presents results from the following paper:
\begin{adjustwidth}{.1\textwidth}{.1\textwidth}
{
\vspace{1em}
\setlength{\parindent}{0pt}
\bibentry{brandt_grunau_rozhon2020tightLLL}
\vspace{1em}
}
\end{adjustwidth}

\cref{chap:8speedup_logstar} presents results from the following paper:
\begin{adjustwidth}{.1\textwidth}{.1\textwidth}
{
\vspace{1em}
\setlength{\parindent}{0pt}
\bibentry{grunau_rozhon_brandt2022speedups_below_log_star}
\vspace{1em}
}    
\end{adjustwidth}



The remaining \cref{chap:9volume_lll,chap:10parallel_decomposition,chap:11trees_descriptive} can be seen as applying the principles and techniques of local algorithms to other related areas. 

%\cite{rozhon_haeupler_grunau2023simple_decomposition,brandt_grunau_rozhon2020tightLLL,grunau_rozhon_brandt2022speedups_below_log_star,brandt_grunau_rozhon2021LLL_in_LCA,elkin_haeupler_rozhon_grunau2022Clusterings_LSST,brandt_chang_grebik_grunau_rozhon_vidnyanszky2021homomorphism_graphs}:
\cref{chap:9volume_lll} presents results from the following paper:
\begin{adjustwidth}{.1\textwidth}{.1\textwidth}
{
\vspace{1em}
\setlength{\parindent}{0pt}
\bibentry{brandt_grunau_rozhon2021LLL_in_LCA}
\vspace{1em}
}
\end{adjustwidth}
Additionally, \cref{chap:9volume_lll} contains a proof of a result proven in the paper covered in \cref{chap:8speedup_logstar} that more closely fits into the topic of \cref{chap:9volume_lll}. 

\cref{chap:10parallel_decomposition} presents results from the following paper:
\begin{adjustwidth}{.1\textwidth}{.1\textwidth}
{
\vspace{1em}
\setlength{\parindent}{0pt}
\bibentry{elkin_haeupler_rozhon_grunau2022Clusterings_LSST}
\vspace{1em}
}
\end{adjustwidth}

\cref{chap:11trees_descriptive} presents results from the following paper:
\begin{adjustwidth}{.1\textwidth}{.1\textwidth}
{
\vspace{1em}
\setlength{\parindent}{0pt}
\bibentry{brandt_chang_grebik_grunau_rozhon_vidnyanszky2021trees}
\vspace{1em}
}
\end{adjustwidth}

During his doctoral studies, the author has also coauthored other papers related to the local/distributed/parallel algorithms \cite{ghaffari_grunau_rozhon2020improved_network_decomposition,
grebik_rozhon2021paths,
grebik_rozhon2023grids,
brandt_chang_grebik_grunau_rozhon_vidnyanszky2021homomorphism_graphs,
rozhon_grunau_haeupler_zuzic_li2022deterministic_sssp,
bezdrighin2022deterministic,
faour2023local,
ghaffari_grunau_haeupler_ilchi_rozhon2023improved_decomposition,
rozhon_haeupler_martinsson_grunau2023parallel_sssp,
ghaffari_grunau_rozhon2023work_efficient_derandomization} and some other papers \cite{choo2020k,
rozhon2020simple,grunau_rozhon2020adapting_kmeans_to_outliers,
grunau_ozudogru_rozhon_tetek2023nearly_tight_kmeans,lacki_hauepler_gruanu_rozhon2023fully_dynamic_consistent_kcenter,
grunau_ozudogru_rozhon2023noisy_kmeans,
haeupler_hladik_rozhon_tarjan_tetek2023universal_dijkstra,
grebik_greenfeld_rozhon_tao2023measurable}. 

